Data-Aware Socratic Query Refinement in Database Systems

In this paper, we propose Data-Aware Socratic Guidance (DASG), a dialogue-based query enhancement framework that embeds \linebreak interactive clarification as a first-class operator within database systems to resolve ambiguity in natural language queries. DASG treats dialogue as an optimization decision, asking clarifying questions only when the expected execution cost reduction exceeds the interaction overhead. The system quantifies ambiguity through linguistic fuzziness, schema grounding confidence, and projected costs across relational and vector backends. Our algorithm selects the optimal clarifications by combining semantic relevance, catalog-based information gain, and potential cost reduction. We evaluate our proposed framework on three datasets. The results show that DASG demonstrates improved query precision while maintaining efficiency, establishing a cooperative analytics paradigm where systems actively participate in query formulation rather than passively translating user requests.

==> MIU.tex <==
This section presents the MIU algorithm in detail. The ranker implements a scoring-based selection procedure over candidate facets. Each score incorporates semantic, statistical, and cost-based signals to compute an overall utility.


\begin{algorithm}[h]
\caption{Maximum Information Utility (MIU) Ranker}
\label{alg:miu}
\begin{algorithmic}[1]
\Require Query $q$, candidate facets $F = \{f_1, \dots, f_n\}$, database context $C$
\Ensure Selected facet $f^*$
\For{each facet $f_i \in F$}
    \State $S_{\text{rel}} \gets$ \Call{SemanticRelevance}{$q, f_i$}
    \State $S_{\text{ig}} \gets$ \Call{EstimatedInfoGain}{$f_i, C$}
    \State $S_{\text{cost}} \gets$ \Call{EstimatedEvalCost}{$f_i, C$}
    \State $\text{MIU\_Score}(f_i) \gets \alpha \cdot S_{\text{rel}} + \beta \cdot S_{\text{ig}} - \gamma \cdot S_{\text{cost}}$
\EndFor
\State \Return $f^* \gets \arg\max_{f_i \in F} \text{MIU\_Score}(f_i)$
\end{algorithmic}
\end{algorithm}


For facet $i$ the utility score is a weighted sum of three terms:

\begin{enumerate}
    \item \textbf{Semantic relevance $S_i$}
    A sentence-embedding model measures the cosine similarity between the user’s request and the facet’s textual description—table or column name plus any catalog comment. A high value indicates that the facet is likely to match the user’s intent.
    \item \textbf{Information gain} $G_i$
    The optimizer consults histograms or vector-index summaries to estimate the entropy of the current result set and of the set that would remain if facet i were fixed to a single value. The relative drop in entropy is the expected reduction in uncertainty.
    \item \textbf{Cost reduction} $C_i$
    The system injects facet $i$ into the provisional query and issues an \texttt{EXPLAIN}. The fraction by which the reported plan cost falls, relative to the original, is the anticipated saving in I/O, CPU, or GPU work. 
\end{enumerate}


\subsection{Semantic Relevance ($S_{\text{rel}}$)}

We compute the semantic relevance of each facet to the user query using cosine similarity in a shared embedding space:
\[
S_{\text{rel}}(f_i) = \cos(\text{Embed}(q), \text{Embed}(f_i))
\]
Embeddings are obtained from a pre-trained language model such as BERT. This score captures linguistic proximity and ensures that suggested questions remain contextually aligned.

\subsection{Information Gain ($S_{\text{ig}}$)}

We estimate the expected information gain of a facet based on entropy reduction:
\[
S_{\text{ig}}(f_i) = \frac{H(R) - H(R \mid f_i)}{H(R)}
\]
where $H(R)$ is the entropy of the candidate result set before applying the facet, and $H(R \mid f_i)$ is the entropy after applying it. In practice:
\begin{itemize}
    \item For structured data, we approximate entropy using cardinality and selectivity statistics.
    \item For vector data, we estimate local density using techniques such as relative contrast or LID.
\end{itemize}

\subsection{Evaluation Cost ($S_{\text{cost}}$)}

The cost score reflects the estimated overhead of executing the query with the facet applied:
\[
S_{\text{cost}}(f_i) = \text{EstCost}(f_i)
\]
We normalize this value to $[0, 1]$ based on typical system profiles. For relational data, cost is estimated using access path statistics. For vector search, we model the expected number of index probes and distance computations under the current indexing strategy (e.g., HNSW or IVF).

\subsection{Final Utility Score}

Each facet is scored using a weighted combination of the three signals:
\[
\text{MIU\_Score}(f_i) = \alpha \cdot S_{\text{rel}}(f_i) + \beta \cdot S_{\text{ig}}(f_i) - \gamma \cdot S_{\text{cost}}(f_i)
\]
Weights $\alpha$, $\beta$, and $\gamma$ are system-tunable. In our deployment, we found that prioritizing information gain ($\beta > \alpha$) yielded better overall interaction quality.

\subsection{Implementation Notes}

The MIU Ranker uses backend-specific evaluators to compute scores in both relational and vector systems. Common facet types are cached to reduce per-query overhead. The algorithm is stateless and can be executed independently for each incoming query.
